AI-EDI-SPACE: A Co-designed Dataset for Evaluating the Quality of Public Spaces

Advancements in AI heavily rely on large-scale datasets meticulously curated and annotated for training. However, concerns persist regarding the transparency and context of data collection methodologies, especially when sourced through crowdsourcing platforms. Crowdsourcing often employs low-wage workers with poor working conditions and lacks consideration for the representativeness of annotators, leading to algorithms that fail to represent diverse views and perpetuate biases against certain groups. To address these limitations, we propose a methodology involving a co-design model that actively engages stakeholders at key stages, integrating principles of Equity, Diversity, and Inclusion (EDI) to ensure diverse viewpoints. We apply this methodology to develop a dataset and AI model for evaluating public space quality using street view images, demonstrating its effectiveness in capturing diverse perspectives and fostering higher-quality data.

==> sec/6_future.tex <==
\section{Plausible Solutions}
\label{solutions}
In our study, we also discuss plausible solutions to increase the equity over the participants’ domain in an LTR task. 
We discuss pre-processing techniques like scaling and normalisation, which ensures sparse unanimity, and also discuss in-processing techniques like using user embeddings and specific loss functions to ensure that the algorithm learns users’ voting patterns. 

\subsection{Pre-Processing Techniques}
Pre-processing techniques are used to pre-process the data before training the algorithm on it. 
Scaling can be done to equalise the voting patterns of the participants. 
In this study, we experiment with Min-Max Scaling, Normalisation Scaling, and Mehestan Scaling \cite{allouah_robust_2022}. 
Min-max scaling and Normalisation scaling are individual-based scaling algorithms which do not guarantee sparse unanimity \cite{allouah_robust_2022}. 
For min-max scaling, we scale the scores given by every participant such that their maximum value is one and minimum value is -1. 
This is done over all the scores of the same participant and then iterated over all participants. 
For normalisation scaling, we first perform a standard normalisation and make the mean and standard deviation of all scores from a participant to 0 and 1, respectively.
To add homogeneity, we then scale the values such that they remain between -1 and 1.
Mehestan is a collaborative score scaling approach which uses the voting patterns of other participants to scale the scores from a single participant.
For mehestan scaling, we first convert the scores from raw comparisons to individual scores using a Generalised Bradley-Terry Model \cite{fageot_generalized_2023}.
This is a probabilistic model that predicts the distribution of the participant’s score.
After we get the raw scores, we scale and translate them using a primitive called BrMean \cite{allouah_robust_2022}, which is resilient to malicious voters who poison the ranking.
It is also helpful for sparse unanimity.
We do not aggregate the data as is done in the last step of the Mehestan algorithm, as we wish to keep the scores by participants separate and individual.
The results of all experiments can be seen in Table \ref{sol_results}. More detailed results can be found in Appendix B.

\subsection{In-Processing Techniques}

In-processing techniques are used while the algorithm is training.
We use User embedding to make the model learn the different participant voting patterns.
We also use Contrastive loss along with LSE.
Contrastive loss \cite{noauthor_contrastive_nodate} is a type of loss which tries to increase the distance between dissimilar scores.
Our use of contrastive loss is to make sure the output of the models is not clustered so that the comparisons, which are simply the subtraction of scores of the two alternatives, do not have a score very close to 0.
These results can be seen in Table \ref{sol_results}.

\begin{table*}[t]
\caption{Results of our metrics over different plausible solutions}
\label{sol_results}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccr}
\toprule
Name of Experiment & Accuracy & Maximal Per-User Accuracy  & Standard Deviation of Per-User Accuracy & Recall & Maximal Per-User Recall  & Standard Deviation of Per-User Recall   \\
\midrule
Baseline & 47.97\%   & 7.43\%    & 2.01\%    & 48.10\%   & 9.45\%    & 2.10\% \\
Contrastive Loss & 50.31\%   & 7.88\%    & 1.75\%    & 51.19\%   & 15.47\%    & 3.34\% \\
Min-Max scaling & 49.26\%   & 10.04\%    & 2.45\%    & 48.87\%   & 14.12\%    & 3.48\% \\
Min-Max + Contrastive Loss & \textbf{51.40\%}   & 5.94\%    & 1.71\%    & \textbf{51.98\%}   & 13.65\%    & 2.73\% \\
Normalisation scaling & 48.82\%   & 14.65\%    & 2.62\%    & 48.08\%   & 10.57\%    & 2.45\% \\
Normalisation + Contrastive Loss & 49.45\%   & 7.12\%    & 1.62\%    & 49.58\%   & 9.38\%    & 2.17\% \\
Mehestan scaling & 48.82\%   & 6.76\%    & 1.85\%    & 49.07\%   & 9.01\%    & 2.13\% \\
Mehestan + Contrastive loss & 50.49\%   & 9.29\%    & 2.18\%    & 51.65\%   & 8.78\%    & 2.29\% \\
User Embeddings & 49.67\%   & 5.47\%    & 1.43\%    & 49.72\%   & \textbf{6.92\%}    & \textbf{1.89\%} \\ 
User Embeddings + Contrastive Loss & 49.93\%   & \textbf{4.68\%}    & \textbf{1.08\%}    & 50.10\%   & 8.01\%    & 2.00\% \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

